Machine learning-based malware detection for IoT devices using control-flow data

Embedded devices are specialised devices designed for one or only a few purposes. They are often part of a larger system, through wired or wireless connection. Those embedded devices that are connected to other computers or embedded systems through the Internet are called Internet of Things (IoT for short) devices. With their widespread usage and their insufficient protection, these devices are increasingly becoming the target of malware attacks. Companies often cut corners to save manufacturing costs or misconfigure when producing these devices. This can be lack of software updates, ports left open or security defects by design. Although these devices may not be as powerful as a regular computer, their large number makes them suitable candidates for botnets. Other types of IoT devices can even cause health problems since there are even pacemakers connected to the Internet. This means, that without sufficient defence, even directed assaults are possible against people. The goal of this thesis project is to provide better security for these devices with the help of machine learning algorithms and reverse engineering tools. Specifically, I study the applicability of control-flow related data of executables for malware detection. I present a malware detection method with two phases. The first phase extracts control-flow related data using static binary analysis. The second phase classifies binary executables as either malicious or benign using a neural network model. I train the model using a dataset of malicious and benign ARM applications.

==> Makefile <==
DOCUMENT=thesis
#MODE=-interaction=batchmode

all: clean xelatex
	echo

xelatex: compile_xelatex
	mv $(DOCUMENT)-xelatex.pdf ../pdf/$(DOCUMENT).pdf

compile_xelatex:
	xelatex $(MODE) $(DOCUMENT)
	bibtex $(DOCUMENT)
	xelatex $(MODE) $(DOCUMENT)
	xelatex $(MODE) $(DOCUMENT)
	mv $(DOCUMENT).pdf $(DOCUMENT)-xelatex.pdf

pdflatex: compile_pdflatex
	mv $(DOCUMENT)-pdflatex.pdf ../pdf/$(DOCUMENT).pdf

compile_pdflatex:
	pdflatex $(MODE) $(DOCUMENT)
	bibtex $(DOCUMENT)
	pdflatex $(MODE) $(DOCUMENT)
	pdflatex $(MODE) $(DOCUMENT)
	mv $(DOCUMENT).pdf $(DOCUMENT)-pdflatex.pdf

lualatex: compile_lualatex
	mv $(DOCUMENT)-lualatex.pdf ../pdf/$(DOCUMENT).pdf

compile_lualatex:
	lualatex $(MODE) $(DOCUMENT)
	bibtex $(DOCUMENT)
	lualatex $(MODE) $(DOCUMENT)
	lualatex $(MODE) $(DOCUMENT)
	mv $(DOCUMENT).pdf $(DOCUMENT)-lualatex.pdf

switch_to_hungarian:
	sed -i "s|^\\\input{include/thesis-en}|%\\\input{include/thesis-en}|" $(DOCUMENT).tex
	sed -i "s|^%\\\input{include/thesis-hu}|\\\input{include/thesis-hu}|" $(DOCUMENT).tex

test_hu:
	${MAKE} clean compile_xelatex
	${MAKE} clean compile_pdflatex
	${MAKE} clean compile_lualatex
	mv $(DOCUMENT)-xelatex.pdf ../pdf/$(DOCUMENT)-xelatex-hu.pdf
	mv $(DOCUMENT)-pdflatex.pdf ../pdf/$(DOCUMENT)-pdflatex-hu.pdf
	mv $(DOCUMENT)-lualatex.pdf ../pdf/$(DOCUMENT)-lualatex-hu.pdf

switch_to_english:
	sed -i "s|^\\\input{include/thesis-hu}|%\\\input{include/thesis-hu}|" $(DOCUMENT).tex
	sed -i "s|^%\\\input{include/thesis-en}|\\\input{include/thesis-en}|" $(DOCUMENT).tex

test_en:
	${MAKE} switch_to_english
	${MAKE} clean compile_xelatex
	${MAKE} clean compile_pdflatex
	${MAKE} clean compile_lualatex
	mv $(DOCUMENT)-xelatex.pdf ../pdf/$(DOCUMENT)-xelatex-en.pdf
	mv $(DOCUMENT)-pdflatex.pdf ../pdf/$(DOCUMENT)-pdflatex-en.pdf
	mv $(DOCUMENT)-lualatex.pdf ../pdf/$(DOCUMENT)-lualatex-en.pdf
	${MAKE} switch_to_hungarian

test: test_hu test_en
	echo

clean:
	echo Cleaning temporary files...
	rm -f *.aux *.dvi *.thm *.lof *.log *.lot *.fls *.out *.toc *.bbl *.blg


==> content/appendices.tex <==
%----------------------------------------------------------------------------
\appendix
%----------------------------------------------------------------------------
\chapter*{\fuggelek}\addcontentsline{toc}{chapter}{\fuggelek}
\setcounter{chapter}{\appendixnumber}
%\setcounter{equation}{0} % a fofejezet-szamlalo az angol ABC 6. betuje (F) lesz
\numberwithin{equation}{section}
\numberwithin{figure}{section}
\numberwithin{lstlisting}{section}
%\numberwithin{tabular}{section}



==> content/latex-tools.tex <==
%----------------------------------------------------------------------------
\chapter{\LaTeX-eszközök}
\label{sec:LatexTools}
%----------------------------------------------------------------------------
\section{A szerkesztéshez használatos eszközök}
%----------------------------------------------------------------------------
Ez a sablon TeXstudio 2.8.8 szerkesztővel készült. A TeXstudio egy platformfüggetlen, Windows, Linux és Mac OS alatt is elérhető \LaTeX-szerkesztőprogram számtalan hasznos szolgáltatással (\refstruc{fig:TeXstudio}). A szoftver ingyenesen letölthető\footnote{A TeXstudio hivatalos oldala: \url{http://texstudio.sourceforge.net/}}.

\begin{figure}[!ht]
\centering
\includegraphics[width=150mm, keepaspectratio]{figures/TeXstudio.png}
\caption{A TeXstudio \LaTeX-szerkesztő.}
\label{fig:TeXstudio}
\end{figure}

A TeXstudio telepítése után érdemes még letölteni a magyar nyelvű helyesírásellenőrző-szótárakat hozzá. A TeXstudio az OpenOffice-hoz használatos formátumot tudja kezelni. A TeXstudio beállításainál a \verb+General+ fülön a \verb+Dictionaries+ résznél tudjuk megadni, hogy melyik szótárat használja.

Egy másik használható Windows alapú szerkesztőprogram a LEd\footnote{A LEd hivatalos oldala: \url{http://www.latexeditor.org/}} (LaTeX Editor), a TeXstudio azonban stabilabb, gyorsabb, és jobban használható.

%----------------------------------------------------------------------------
\section{A dokumentum lefordítása Windows alatt}
%----------------------------------------------------------------------------
A TeXstudio és a LEd kizárólag szerkesztőprogram (bár az utóbbiban DVI-nézegető is van), így a dokumentum fordításához szükséges eszközöket nem tartalmazza. Windows alatt alapvetően két lehetőség közül érdemes választani: MiKTeX (\url{http://miktex.org/}) és TeX Live (\url{http://www.tug.org/texlive/}) programcsomag. Az utóbbi működik Mac OS X, GNU/Linux alatt és Unix-származékokon is. A MiKTeX egy alapcsomag telepítése után mindig letölti a használt funkciókhoz szükséges, de lokálisan hiányzó \TeX-csomagokat, míg a TeX Live DVD ISO verzóban férhető hozzá. Ez a dokumentum TeX Live 2008 programcsomag segítségével fordult, amelynek DVD ISO verziója a megadott oldalról letölthető. A sablon lefordításához a disztribúcióban szereplő \verb+magyar.ldf+ fájlt a \verb+http://www.math.bme.hu/latex/+ változatra kell cserélni, vagy az utóbbi változatot be kell másolni a projekt-könyvtárba (ahogy ezt meg is tettük a sablonban) különben anomáliák tapasztalhatók a dokumentumban (pl. az ábra- és táblázat-aláírások formátuma nem a beállított lesz, vagy bizonyos oldalakon megjelenik alapértelmezésben egy fejléc). A TeX Live 2008-at még nem kell külön telepíteni a gépre, elegendő DVD-ről (vagy az ISO fájlból közvetlenül, pl. DaemonTools-szal) használni.

Ha a MiKTeX csomagot használjuk, akkor parancssorból a következő módon tudjuk újrafordítani a teljes dokumentumot:

\begin{lstlisting}[language=bash,frame=single,float=!ht]
$ texify -p thesis.tex
\end{lstlisting}

A \verb+texify+ parancs a MiKTex programcsomag \verb+miktex/bin+ alkönyvtárában található. A parancs gondoskodik arról, hogy a szükséges lépéseket (fordítás, hivatkozások generálása stb.) a megfelelő sorrendben elvégezze. A \verb+-p+ kapcsoló hatására PDF-et generál. A fordítást és az ideiglenes fájlok törlését elvégezhetjük a sablonhoz mellékelt \verb+manual_build.bat+ szkript segítségével is.

A \TeX-eszközöket tartalmazó programcsomag binárisainak elérési útját gyakran be kell állítani a szerkesztőprogramban, például TeXstudio esetén legegyszerűbben az \verb+Options / Configure TeXstudio... / Commands+ menüponttal előhívott dialógusablakban tehetjük ezt meg.

A PDF-\LaTeX~használata esetén a generált dokumentum közvetlenül PDF-formátumban áll rendelkezésre. Amennyiben a PDF-fájl egy PDF-nézőben (pl. Adobe Acrobat Reader vagy Foxit PDF Reader) meg van nyitva, akkor a fájlleírót a PDF-néző program tipikusan lefoglalja. Ilyen esetben a dokumentum újrafordítása hibaüzenettel kilép. Ha bezárjuk és újra megnyitjuk a PDF dokumentumot, akkor pedig a PDF-nézők többsége az első oldalon nyitja meg a dokumentumot, nem a legutóbb olvasott oldalon. Ezzel szemben például az egyszerű és ingyenes \textcolor{blue}{Sumatra PDF} nevű program képes arra, hogy a megnyitott dokumentum megváltozását detektálja, és frissítse a nézetet az aktuális oldal megtartásával.

%----------------------------------------------------------------------------
\section{Eszközök Linuxhoz}
%----------------------------------------------------------------------------
Linux operációs rendszer alatt is rengeteg szerkesztőprogram van, pl. a KDE alapú Kile jól használható. Ez ingyenesen letölthető, vagy éppenséggel az adott Linux-disztribúció eleve tartalmazza, ahogyan a dokumentum fordításához szükséges csomagokat is. Az Ubuntu Linux disztribúciók alatt például legtöbbször a \verb+texlive-*+ csomagok telepítésével használhatók a \LaTeX-eszközök. A jelen sablon fordításához szükséges csomagok (kb. 0,5 GB) az alábbi paranccsal telepíthetők:

\begin{lstlisting}[language=bash,morekeywords={sudo,apt\-get},alsoletter={-},breaklines=true]
$ sudo apt-get install texlive-latex-extra texlive-fonts-extra texlive-fonts-recommended texlive-xetex texlive-science
\end{lstlisting}

Amennyiben egy újabb csomag hozzáadása után hiányzó fájlra utaló hibát kapunk a fordítótól, telepítenünk kell az azt tartalmazó TeX Live csomagot. Ha pl. a \verb+bibentry+ csomagot szeretnénk használni, futtassuk az alábbi parancsot:

\begin{lstlisting}[language=bash,morekeywords={apt\-cache},alsoletter={-},breaklines=true]
$ apt-cache search bibentry
texlive-luatex - TeX Live: LuaTeX packages
\end{lstlisting}

Majd telepítsük fel a megfelelő TeX Live csomagot, jelen esetben a `texlive-lualatex`-et. (Egy LaTeX csomag több TeX Live csomagban is szerepelhet.)

Ha gyakran szerkesztünk más \LaTeX dokumentumokat is, kényelmes és biztos megoldás a teljes TeX Live disztribúció telepítése, ez azonban kb. 4 GB helyet igényel.

\begin{lstlisting}[language=bash,morekeywords={sudo,apt\-get},alsoletter={-},breaklines=true]
sudo apt-get install texlive-full
\end{lstlisting}


==> content/thesis-format.tex <==
%----------------------------------------------------------------------------
\chapter{A dolgozat formai kivitele}
%----------------------------------------------------------------------------
Az itt található információk egy része a BME VIK Hallgatói Képviselet által készített ,,Utolsó félév a villanykaron'' c. munkából lett kis változtatásokkal átemelve. Az eredeti dokumentum az alábbi linken érhető el: \url{http://vik.hk/hirek/diplomafelev-howto-2015}.

%----------------------------------------------------------------------------
\section{A dolgozat kimérete}
%----------------------------------------------------------------------------
Szakdolgozat esetében minimum 30, 45 körüli ajánlott oldalszám lehet az iránymutató. De mindenképp érdemes rákérdezni a konzulensnél is az elvárásokra, mert tanszékenként változóak lehetnek az elvárások.

Mesterképzésen a Diplomatervezés 1 esetében a beszámoló még inkább az Önálló laboratóriumi beszámolókhoz hasonlít, tanszékenként eltérő formai követelményekkel, -- egy legalább 30 oldal körüli dolgozat az elvárt -- és az elmúlt fél éves munkáról szól. De egyben célszerű, ha ez a végleges diplomaterv alapja is. (A végleges 60-90 oldal körülbelül a hasznos részre nézve)


%----------------------------------------------------------------------------
\section{A dolgozat nyelve}
%----------------------------------------------------------------------------
Mivel Magyarországon a hivatalos nyelv a magyar, ezért alapértelmezésben magyarul kell megírni a dolgozatot. Aki külföldi posztgraduális képzésben akar részt venni, nemzetközi szintű tudományos kutatást szeretne végezni, vagy multinacionális cégnél akar elhelyezkedni, annak célszerű angolul megírnia diplomadolgozatát. Mielőtt a hallgató az angol nyelvű verzió mellett dönt, erősen ajánlott mérlegelni, hogy ez mennyi többletmunkát fog a hallgatónak jelenteni fogalmazás és nyelvhelyesség terén, valamint -- nem utolsó sorban -- hogy ez mennyi többletmunkát fog jelenteni a konzulens illetve bíráló számára. Egy nehezen olvasható, netalán érthetetlen szöveg teher minden játékos számára.

%----------------------------------------------------------------------------
\section{A dokumentum nyomdatechnikai kivitele}
%----------------------------------------------------------------------------
A dolgozatot A4-es fehér lapra nyomtatva, 2,5 centiméteres margóval (+1~cm kötésbeni), 11--12 pontos betűmérettel, talpas betűtípussal és másfeles sorközzel célszerű elkészíteni.

Annak érdekében, hogy a dolgozat külsőleg is igényes munka benyomását keltse, érdemes figyelni az alapvető tipográfiai szabályok betartására~\cite{Jeney}.


==> include/project.tex <==
%--------------------------------------------------------------------------------------
% Feladatkiiras (a tanszeken atveheto, kinyomtatott valtozat)
%--------------------------------------------------------------------------------------
\clearpage
\begin{center}
\large
\textbf{FELADATKIÍRÁS}\\
\end{center}

A feladatkiírást a tanszéki adminisztrációban lehet átvenni, és a leadott munkába eredeti, tanszéki pecséttel ellátott és a tanszékvezető által aláírt lapot kell belefűzni (ezen oldal \emph{helyett}, ez az oldal csak útmutatás). Az elektronikusan feltöltött dolgozatban már nem kell beleszerkeszteni ezt a feladatkiírást.


==> include/tdk-variables.tex <==
%--------------------------------------------------------------------------------------
% TDK-specifikus változók
%--------------------------------------------------------------------------------------
\newcommand{\tdkszerzoB}{Második Szerző} % Második szerző neve; hagyd üresen, ha egyedül írtad a TDK-t.
\newcommand{\tdkev}{2014} % A dolgozat írásának éve (pl. "2014") (Ez OTDK-nál eltérhet az aktuális évtől.)

% További adatok az OTDK címlaphoz (BME-s TDK-hoz nem kell kitölteni)
\newcommand{\tdkevfolyamA}{IV} % Első szerző évfolyama, római számmal (pl. IV).
\newcommand{\tdkevfolyamB}{III} % Második szerző évfolyama, római számmal (pl. III).
\newcommand{\tdkkonzulensbeosztasA}{egyetemi tanár} % Első konzulens beosztása (pl. egyetemi docens)
\newcommand{\tdkkonzulensbeosztasB}{doktorandusz} % Második konzulens beosztása (pl. egyetemi docens)


==> include/thesis-hu.tex <==
%--------------------------------------------------------------------------------------
% Elnevezések
%--------------------------------------------------------------------------------------
\newcommand{\bme}{Budapesti Műszaki és Gazdaságtudományi Egyetem}
\newcommand{\vik}{Villamosmérnöki és Informatikai Kar}

\newcommand{\bmemit}{Méréstechnika és Információs Rendszerek Tanszék}

\newcommand{\keszitette}{Készítette}
\newcommand{\konzulens}{Konzulens}

\newcommand{\bsc}{Szakdolgozat}
\newcommand{\msc}{Diplomaterv}
\newcommand{\tdk}{TDK dolgozat}
\newcommand{\bsconlab}{BSc Önálló laboratórium}
\newcommand{\msconlabi}{MSc Önálló laboratórium 1.}
\newcommand{\msconlabii}{MSc Önálló laboratórium 2.}

\newcommand{\pelda}{Példa}
\newcommand{\definicio}{Definíció}
\newcommand{\tetel}{Tétel}

\newcommand{\bevezetes}{Bevezetés}
\newcommand{\koszonetnyilvanitas}{Köszönetnyilvánítás}
\newcommand{\fuggelek}{Függelék}

% Opcionálisan átnevezhető címek
%\addto\captionsmagyar{%
%\renewcommand{\listfigurename}{Saját ábrajegyzék cím}
%\renewcommand{\listtablename}{Saját táblázatjegyzék cím}
%\renewcommand{\bibname}{Saját irodalomjegyzék név}
%}

\newcommand{\szerzo}{\vikszerzoVezeteknev{} \vikszerzoKeresztnev}
\newcommand{\vikkonzulensA}{\vikkonzulensAMegszolitas\vikkonzulensAVezeteknev{} \vikkonzulensAKeresztnev}
\newcommand{\vikkonzulensB}{\vikkonzulensBMegszolitas\vikkonzulensBVezeteknev{} \vikkonzulensBKeresztnev}
\newcommand{\vikkonzulensC}{\vikkonzulensCMegszolitas\vikkonzulensCVezeteknev{} \vikkonzulensCKeresztnev}

\newcommand{\selectthesislanguage}{\selecthungarian}

\bibliographystyle{huplain}

\def\lstlistingname{lista}

\newcommand{\appendixnumber}{6}  % a fofejezet-szamlalo az angol ABC 6. betuje (F) lesz


==> include/titlepage-tdk.tex <==
%% TDK címlap
\begin{titlepage}
  \begin{center}  
  \includegraphics[width=7cm]{./figures/bme_logo.pdf}
  \vspace{0.3cm}
  
  \bme \\
  \vik \\
  \viktanszek \\
  \vspace{5cm}
  
  \huge {\vikcim}
  \vspace{1.5cm}
  
  \large {\textbf{\tdk}}
  \vfill
    
  {\Large 
  	\keszitette: \\ \vspace{0.3cm}
  	\szerzo \\
	\tdkszerzoB \\
  	\vspace{1.5cm}
  	\konzulens: \\ \vspace{0.3cm}
  	\vikkonzulensA \\
  	\vikkonzulensB \\
  }
  
  \vspace{2cm}
  \large {\tdkev}
 \end{center}
\end{titlepage}
%% Címlap vége

